Sobolev GAN

We propose a new Integral Probability Metric (IPM) between distributions: the Sobolev IPM. The Sobolev IPM compares the mean discrepancy of two distributions for functions (critic) restricted to a Sobolev ball defined with respect to a dominant measure $\mu$. We show that the Sobolev IPM compares two distributions in high dimensions based on weighted conditional Cumulative Distribution Functions (CDF) of each coordinate on a leave one out basis. The Dominant measure $\mu$ plays a crucial role as it defines the support on which conditional CDFs are compared. Sobolev IPM can be seen as an extension of the one dimensional Von-Mises Cram\'er statistics to high dimensional distributions. We show how Sobolev IPM can be used to train Generative Adversarial Networks (GANs). We then exploit the intrinsic conditioning implied by Sobolev IPM in text generation. Finally we show that a variant of Sobolev GAN achieves competitive results in semi-supervised learning on CIFAR-10, thanks to the smoothness enforced on the critic by Sobolev GAN which relates to Laplacian regularization.

==> NOTE <==
# Oct 29 Ideas while writing the empirical paper.
in comparison with WGAN-GP,
add a remark that
(1) the main difference is that our formulation allows the theory,
(2) we step away from the lipschitzity argument
(3) empirically the sample-wise constraint with high lambda really forces all those gradient norms to 1,
    somehow "harsher" constraint. so our ALM sobolev allows more flexibility during early training


Stress more the difference between tractable & intractable function classes \F.
+ intractable: lipschitz constraint. Needs HACKY APPROXIMATIONS (clipping, gp on interpolation).
    clipping is stronger constraint on f than lipschitzity,
    GP on interpolation (even when tight) is weaker constraint??? cause oustide $P,Q$ density it could be non-lipschitz.
+ tractable: mmd, fisher gan, sobolev gan cause constraint defined as function of distributions we can sample from.

Update Fisher GAN  No-norm from 115.

